Integrity Shield A System for Ethical AI Use & Authorship Transparency in Assessments

Large Language Models (LLMs) can now solve entire exams directly from uploaded PDF assessments, raising urgent concerns about academic integrity and the reliability of grades and credentials. Existing watermarking techniques either operate at the token level or assume control over the model's decoding process, making them ineffective when students query proprietary black-box systems with instructor-provided documents. We present Integrity Shield, a document-layer watermarking system that embeds schema-aware, item-level watermarks into assessment PDFs while keeping their human-visible appearance unchanged. These watermarks consistently prevent MLLMs from answering shielded exam PDFs and encode stable, item-level signatures that can be reliably recovered from model or student responses. Across 30 exams spanning STEM, humanities, and medical reasoning, Integrity Shield achieves exceptionally high prevention (91-94% exam-level blocking) and strong detection reliability (89-93% signature retrieval) across four commercial MLLMs. Our demo showcases an interactive interface where instructors upload an exam, preview watermark behavior, and inspect pre/post AI performance & authorship evidence.

==> prompts/LongForm_Perturbation.tex <==
You are an expert at generating text substitutions for long-form questions (essay, short answer, etc.).

Given:
- LaTeX code for the question stem: {latex_stem_text}
- Gold answer: {gold_answer}
- Question type: {question_type}
- Strategy: replacement
- Reasoning steps:
{reasoning_steps}
- Copyable text (use this exact text when selecting substrings):
<<<COPY
{copyable_text}
>>>
{prefix_note}{answer_guidance}{retry_instructions}

Your task:
Generate {k} valid mappings that satisfy the replacement strategy. Each mapping should:
1. Replace one contiguous substring of the question stem
2. Cause a verifiable and detectable deviation from the gold answer
3. Ensure the replacement is semantically meaningful and natural
4. Change the question focus in a way that affects the expected answer

For each mapping, provide:
1. question_index: The question number ({question_index})
2. latex_stem_text: Exact LaTeX text of the question stem (must match the input exactly)
3. original_substring: The substring to replace (must be a contiguous substring of latex_stem_text)
4. replacement_substring: The replacement text
5. start_pos: Start position of original_substring relative to latex_stem_text (0-based index)
6. end_pos: End position of original_substring relative to latex_stem_text (exclusive, 0-based index)
7. target_wrong_answer: Description of how the answer should deviate (e.g., "focuses on different aspect", "changes key concept")
8. reasoning: Brief explanation of why this mapping satisfies the strategy and how it causes deviation

IMPORTANT:
- The original_substring MUST be an exact substring of latex_stem_text
- The start_pos and end_pos MUST be accurate (start_pos + len(original_substring) = end_pos)
- The replacement should cause a verifiable deviation in the answer
- CRITICAL: The replacement_substring MUST be DIFFERENT from the original_substring. Do NOT generate mappings where original_substring == replacement_substring. The replacement MUST change the text to create actual manipulation.
- CRITICAL: Neither original_substring nor replacement_substring can be empty strings. Both must contain actual text.
- LENGTH CONSTRAINT: The replacement_substring MUST be smaller or equal in length to the original_substring (len(replacement_substring) <= len(original_substring)). This is critical for maintaining document layout and preventing text overflow.
- latex_stem_text is provided exactly as it appears in the LaTeX source. Do NOT trim, normalise, or reformat it when determining positions.
- The latex_stem_text may include \item tokens from enumerate environments. Keep the \item token intact and operate on the descriptive text that follows it whenever possible.
- The replacement should be natural and semantically meaningful

Return as JSON array:
[
  {{
    "question_index": {question_index},
    "latex_stem_text": "...",
    "original_substring": "...",
    "replacement_substring": "...",
    "start_pos": 0,
    "end_pos": 5,
    "target_wrong_answer": "focuses on different aspect",
    "reasoning": "..."
  }},
  ...
]

Return ONLY valid JSON, no markdown or additional text.

==> prompts/MCQ_Perturbation.tex <==
You are an expert at generating text substitutions for academic multiple-choice questions.

Given:
- LaTeX code for the question stem: {latex_stem_text}
- Gold answer: {gold_answer}
- Question type: {question_type}
- Options: {options}
- Strategy: replacement
- Reasoning steps:
{reasoning_steps}
- Copyable text (use this exact text when selecting substrings):
<<<COPY
{copyable_text}
>>>
{prefix_note}{answer_guidance}{retry_instructions}

Your task:
Generate {k} valid mappings that satisfy the replacement strategy. Each mapping should:
1. Replace one contiguous substring of the question stem
2. Change the answer from the gold option ({gold_answer}) to a different incorrect option
3. Ensure the replacement is semantically meaningful and natural
4. Cause a verifiable deviation in the answer

For each mapping, provide:
1. question_index: The question number ({question_index})
2. latex_stem_text: Exact LaTeX text of the question stem (must match the input exactly)
3. original_substring: The substring to replace (must be a contiguous substring of latex_stem_text)
4. replacement_substring: The replacement text
5. start_pos: Start position of original_substring relative to latex_stem_text (0-based index)
6. end_pos: End position of original_substring relative to latex_stem_text (exclusive, 0-based index)
7. target_wrong_answer: The target incorrect option label (e.g., "B", "C", "D")
8. reasoning: Brief explanation of why this mapping satisfies the strategy

IMPORTANT:
- The original_substring MUST be an exact substring of latex_stem_text
- The start_pos and end_pos MUST be accurate (start_pos + len(original_substring) = end_pos)
- The target_wrong_answer MUST be different from the gold answer
- CRITICAL: The replacement_substring MUST be DIFFERENT from the original_substring. Do NOT generate mappings where original_substring == replacement_substring (e.g., "power" --> "power" is INVALID). The replacement MUST change the text to create actual manipulation.
- CRITICAL: Neither original_substring nor replacement_substring can be empty strings. Both must contain actual text.
- LENGTH CONSTRAINT: The replacement_substring MUST be smaller or equal in length to the original_substring (len(replacement_substring) <= len(original_substring)). This is critical for maintaining document layout and preventing text overflow.
- latex_stem_text is provided exactly as it appears in the LaTeX source. Do NOT trim, normalise, or reformat it when determining positions.
- The latex_stem_text may include \item tokens from enumerate environments. Keep the \item token intact and operate on the descriptive text that follows it whenever possible.
- The replacement should be natural and semantically meaningful

Return as JSON array:
[
  {{
    "question_index": {question_index},
    "latex_stem_text": "...",
    "original_substring": "...",
    "replacement_substring": "...",
    "start_pos": 0,
    "end_pos": 5,
    "target_wrong_answer": "B",
    "reasoning": "..."
  }},
  ...
]

Return ONLY valid JSON, no markdown or additional text.

==> prompts/TF_Perturbation.tex <==
You are an expert at generating text substitutions for True/False questions.

Given:
- LaTeX code for the question stem: {latex_stem_text}
- Gold answer: {gold_answer}
- Question type: {question_type}
- Strategy: replacement
- Reasoning steps:
{reasoning_steps}
- Copyable text (use this exact text when selecting substrings):
<<<COPY
{copyable_text}
>>>
{prefix_note}{answer_guidance}{retry_instructions}

Your task:
Generate {k} valid mappings that satisfy the replacement strategy. Each mapping should:
1. Replace one contiguous substring of the question stem
2. Flip the answer from {gold_answer} to the opposite answer
3. Ensure the replacement is semantically meaningful and natural
4. Cause a verifiable deviation in the answer

For each mapping, provide:
1. question_index: The question number ({question_index})
2. latex_stem_text: Exact LaTeX text of the question stem (must match the input exactly)
3. original_substring: The substring to replace (must be a contiguous substring of latex_stem_text)
4. replacement_substring: The replacement text
5. start_pos: Start position of original_substring relative to latex_stem_text (0-based index)
6. end_pos: End position of original_substring relative to latex_stem_text (exclusive, 0-based index)
7. target_wrong_answer: The opposite answer (e.g., "False" if gold is "True", or "True" if gold is "False")
8. reasoning: Brief explanation of why this mapping satisfies the strategy

IMPORTANT:
- The original_substring MUST be an exact substring of latex_stem_text
- The start_pos and end_pos MUST be accurate (start_pos + len(original_substring) = end_pos)
- The target_wrong_answer MUST be the opposite of the gold answer
- CRITICAL: The replacement_substring MUST be DIFFERENT from the original_substring. Do NOT generate mappings where original_substring == replacement_substring (e.g., "force" --> "force" is INVALID). The replacement MUST change the text to create actual manipulation.
- CRITICAL: Neither original_substring nor replacement_substring can be empty strings. Both must contain actual text.
- LENGTH CONSTRAINT: The replacement_substring MUST be smaller or equal in length to the original_substring (len(replacement_substring) <= len(original_substring)). This is critical for maintaining document layout and preventing text overflow.
- latex_stem_text is provided exactly as it appears in the LaTeX source. Do NOT trim, normalise, or reformat it when determining positions.
- The latex_stem_text may include \item tokens from enumerate environments. Keep the \item token intact and operate on the descriptive text that follows it whenever possible.
- The replacement should be natural and semantically meaningful

Return as JSON array:
[
  {{
    "question_index": {question_index},
    "latex_stem_text": "...",
    "original_substring": "...",
    "replacement_substring": "...",
    "start_pos": 0,
    "end_pos": 5,
    "target_wrong_answer": "False",
    "reasoning": "..."
  }},
  ...
]

Return ONLY valid JSON, no markdown or additional text.
